Speech and Natural Language Processing Technologies for Pseudo-Pilot Simulator

This paper describes a simple yet efficient repetition-based modular system for speeding up air-traffic controllers (ATCos) training. E.g., a human pilot is still required in EUROCONTROL's ESCAPE lite simulator (see https://www.eurocontrol.int/simulator/escape) during ATCo training. However, this need can be substituted by an automatic system that could act as a pilot. In this paper, we aim to develop and integrate a pseudo-pilot agent into the ATCo training pipeline by merging diverse artificial intelligence (AI) powered modules. The system understands the voice communications issued by the ATCo, and, in turn, it generates a spoken prompt that follows the pilot's phraseology to the initial communication. Our system mainly relies on open-source AI tools and air traffic control (ATC) databases, thus, proving its simplicity and ease of replicability. The overall pipeline is composed of the following: (1) a submodule that receives and pre-processes the input stream of raw audio, (2) an automatic speech recognition (ASR) system that transforms audio into a sequence of words; (3) a high-level ATC-related entity parser, which extracts relevant information from the communication, i.e., callsigns and commands, and finally, (4) a speech synthesizer submodule that generates responses based on the high-level ATC entities previously extracted. Overall, we show that this system could pave the way toward developing a real proof-of-concept pseudo-pilot system. Hence, speeding up the training of ATCos while drastically reducing its overall cost.

==> optional/optionla_modules.tex <==

% ============ OPTIONAL MODULES ============ 
\section{OPTIONAL MODULES}
\label{subsec:optional_submodules}


% ============ OPTIONAL MODULE ============ 
\subsection{Voice Activity Detection and Diarization}

\todo{Saeed, to add something here}

\todo{transform this into an introductorty paragraph}. In some cases, we don't have access to PTT signals i.e., we need to find out who is speaking when? Let's say that we have an input stream of ATC audio, and we would like to extract this information, how we can do it? 
- Implications: this can be useful for large collection and pseudo-annotation of ATC data for training of ASR or NLP modules for ATC. Also, it can be useful to discard data some kind of data i.e. all ATCO data. Also, it can be used to keep records of communications in cases of accidents or incidents., Or simply if someone in the ANSPs wants to review some data for something else. etcetc. 

\todo{This is from the SLT paper. We need to modify and shorten}

On the acoustic level side, latest work has targeted \textbf{end to end neural-based diarization} (EEND). SD and its derivates, e.g., SCD, have also seen the benefits from this trend. For example,~\cite{el2019joint} builds on top of their proposed baseline for SD (ASR and SD are run in parallel and then the output is merged). They perform joint ASR and SD, claiming that word-level DER can be improved up to 15.8\% in cross-domain evaluations. Afterward, the end-to-end neural diarization (EEND) was introduced in~\cite{fujita2019end_free}, where a full SD model is trained jointly to perform extraction and clustering. Later, the same authors upgraded the system by replacing the bidirectional long short-term memory (BLSTM) layers by self-attention modules~\cite{fujita2019end}. Subsequent work has targeted EEND for long conversations~\cite{mao2020speech} (for example, long stream of ATC audio), streaming EEND~\cite{han2021bw} (for example for deployment in a real ATC room) or even performing EEND and ASR simultaneously~\cite{khare2022asr}.


% ============ OPTIONAL MODULE ============ 
\subsection{Speaker Role Identification}


\todo{We can add/complement here with speaker role paper... Maybe the grammar one. We need to change this paragraph top only speaker role detection.}

On the text level side, Early text-based techniques for SRD or SCD relied on handcrafted lexicons, dictionaries, and rules. They are prone to human errors and not robust against noisy labels, e.g., produced by standard ASR systems. 
Collobert et al.~\cite{collobert2011natural} introduced machine learning methods for text processing in part-of-speech tagging, chunking, and semantic role labeling. 
In~\cite{mohapatra10domain}, domain-based chunking of sentences is addressed, which is similar to the approach proposed in this paper. 
In general, chunking is used to parse phrases from unstructured text e.g., in our case tagging and chunking an ATC utterance (i.e., detect speaker changes and its speaker roles).
The reader might relate chunking to named entity recognition (NER). NER is a chunking sub-task that aims at identifying entities on text, e.g., locations, organizations, or names~\cite{yadav2018survey,sharma2022named}. Examples of named entities in ATC communications are \textit{callsigns}, \textit{command types}, etc. These entities carry rich information that gives cues about the speaker's role (ATCO or pilot). A recent work aligned to ATC domain is reviewed in~\cite{prasad2021grammar}. Here, a grammar-based approach performs SRD on single-speaker utterances. Finally, text-based diarization has been proposed in the past by~\cite{han2021bw,khare2022asr}. However, most of the previous work still relies on developing and training an acoustic-based system that does not take into account the text structure and its grammar. 

\begin{figure}[t]
  \centering
%   \includegraphics[width=0.9\linewidth]{figures/ner_pipeline.png}
  \caption{\todo{make a figure similar to the one on SLT paper}. Proposed approach for text-based speaker role identification based on a BERT-module.}
  \label{fig:speaker_role}
\end{figure}

\todo{update}\textbf{Databases:} In this task. we experiment on three databases in the English language with various accents and data quality. With the aim of encouraging open research on ATC (which has lagged behind due to privacy clauses and contracts\footnote{Nearly all ongoing and former projects in the area of ATC prohibit the release of code and models due to privacy issues.}) we only present experiments with open-source databases, as referenced in Table~\ref{tab:test_sets}. All experiments use 10\% of the train set as validation set.

ATCC, UWB and ATCO2 databases also provide speaker labels and time segmentation\footnote{In other words, we know exactly `who is talking and when'; either ATCO pilot or mixed case (both).} in addition to manual speech transcriptions. We invite the reader to our previous publication for more details on both, the acoustic and text based SD system: citations~\cite{zuluaga2021bertraffic}.

% In case is neccesary we can add information from this apragrpah:
%The BERT model starts by tagging each word of the transcript (ground truth or ASR transcript) with a set of tags that follows the well-known \textit{IOB format} (Inside-Outside-Beginning). In IOB format, each entity (a full sentence in our case) is composed of two tags: (i) the \textit{Beginning} defines which token/word is the start of the sentence \textit{\textbf{`B-'}} and, (ii) the \textit{Inside} tag \textit{\textbf{`I-'}} defines which tokens/words belongs to that specific sentence. We define ATCO recordings as \textit{Speaker1}, while pilot segments as \textit{Speaker2} (green and red in Figure~\ref{fig:diarization_pipeline}, respectively). We do not use the \textit{Outside} tag, because we know that each word is always from one of two predefined speakers. In total, we have four tags, two per each class (ATCO and pilot).

\todo{to update a bit} \textbf{Experimental details:} The SRD system is built on top of a pre-trained BERT\footnote{We use the pre-trained version of \emph{BERT-base-uncased} with 110 million parameters for all the experiments.} model~\cite{devlin-etal-2019-bert} downloaded from HuggingFace~\cite{wolf2020transformers,lhoest2021datasets}. The model is later fine-tuned on the sequence classification task. 
We removed the top layer of the BERT model and replaced it with a linear layer with a dimension of 2 i.e., two-classes, one for ATCO and one for pilot. The experimental hyperparameters follow the exact sames of Section~\ref{subsec:bert_parser}

% these details are the same for NER
%We fine-tune each model on an NVIDIA GeForce RTX 3090 for 10k steps. During experimentation, we use the same learning rate of $\gamma=5\mathrm{e}{-5}$ with a linear learning rate scheduler. Dropout~\cite{srivastava2014dropout} is set to $dp=0.1$ for the attention and hidden layers, while Gaussian Error Linear Units (GELU) is used as activation function~\cite{hendrycks2016gaussian}. We fine-tune each model with an effective batch size of 32 for 50 epochs with AdamW \cite{loshchilov2018decoupled} optimizer ($\beta_1{=}0.9, \beta_2{=}0.999$, $\epsilon{=}1\mathrm{e}{-8}$).


% ============ OPTIONAL MODULE ============ 
\subsection{Contextual Biasing and Personalization}

\todo{This is from boosting paper ICASSP2022, we need to update it}. 
\textbf{Re-ranking module based on Levenshtein distance}: The BERT-based system for NER allows us to extract the callsign from a given transcript or ASR 1-best hypotheses. Recognition of this entity is crucial where a single error produced by the ASR system affects the whole entity (normally composed of three to eight words). Additionally, speakers regularly shorten callsigns in the conversation making it impossible for an ASR system to generate the full entity (e.g., \textit{`three nine two papa'} instead of \textit{`austrian three nine two papa'}, \textit{`six lima yankee'} instead of \textit{`hansa six lima yankee'}). One way to overcome this issue is to re-rank entities extracted by the BERT-based NER system with the surveillance data. The output of an NER system is a list of tags that match words or sequences of words in an input utterance. As our only available source of contextual knowledge are callsigns registered at a certain time and location, we extract callsigns with the NER system and discard other entities. Correspondingly, each utterance has a list of callsigns expanded into word sequences (shown in Table~\ref{tab:callsigns}). As input, the re-ranking module takes (i)~a callsign extracted by the NER system and (ii)~an expanded list of callsigns. The re-ranking module compares a given n-gram sequence against a list of possible n-grams, and finds the closest match from the list of surveillance data based on the weighted Levenshtein distance. In order to use the contextual knowledge, it is necessary to know which words in an utterance correspond to a desired entity (i.e., a callsign), that is why is necessary to add into the pipeline a NER system.
We skip the re-ranking in case the NER system outputs a `NO\_CALLSIGN' flag (no callsign recognized).

\todo{Some work from Yulia's paper ICASSP, we can either run or report results from there.}


\begin{figure}[t]
  \centering
%   \includegraphics[width=0.9\linewidth]{figures/ner_pipeline.png}
  \caption{\todo{make a figure for contextual biasing}. Proposed approach for contextual biasing (or personalization) of the pseudo-pilot module based on real-time surveillance data input.}
  \label{fig:contextual_biasing}
\end{figure}


% ============ OPTIONAL MODULE ============ 
\subsection{PJ16 Parser}
\label{subsec:pj16_parser}

\todo{related work on PJ16 format (basically, some info from )} 

- Information from Hartmut's papers, I can extract something from the paper they're writing now

- Structure, maybe a Figure here and some stats. @Amrutha, you have more info from other docuemtns...

\textbf{Related work:}

\textbf{Our system:}

- We only use a basic grammar-based (string matching) system, one or some words are mapped to one HL entity


==> removed_text.tex <==
%This paper describes a ``repetition-based'' system for training of air-traffic controllers (ATCo). A cascaded system comprising of the following modules is proposes:
The overall pipeline is composed by: 
% We propose a cascade system, where sub-modules are composed of: 
(i) a submodule that receives and pre-processes the input stream of raw audio;
% from ATCos ; 
(ii) an automatic speech recognition (ASR) system that transforms audio to a sequence of words; 
% (iii) a speaker role identification module to verify if the command is issued by an ATCo; 
(iii) a high-level ATC-related entity parser, which extracts relevant information from the communication, for instance, callsigns or commands, 
% (v) a parser module that converts 'relevant' information into PJ16-format alike sentences 
and finally; (iv) a speech synthesizer submodule that generates responses based on the high-level ATC-entities previously extracted. 
In overall, we show that this system could pave the way towards developing a real proof-of-concept pseudo-pilot system. Thus, speeding up the training of ATCos while drastically reducing the overall cost of the ATCO's training pipeline. 

% caption from table 1 
Overall pipeline for simulating a pilot for air traffic controller training. The pipeline starts with an ATCo issuing a communication and its capture via PTT signal. Then, the speech-to-text and high-level parser modules transcribe and extract the ATC-related entities from the voice communication, respectively. The output is then accustomed to 'pilots' structured grammar. The generated textual prompt is then sent to a speech synthesizer module, which generates a WAV file containing the spoken textual prompt. All this together creates a pseudo-pilot that provides pertinent feedback to an ATCo trainee.

Section4 starting
In this section, we describe the core modules of the proposed pseudo-pilot system. The first part cover pre-processing, automatic speech recognition and high-level ATC-entity parsing, as described in Figure~\ref{fig:metadata_pipeline}. These modules will produce the output needed by the speech synthesizer in order to produce the spoken sentence, thus simulating a pilot (second part). An overall overview of the system is in Figure~\ref{fig:full_pipeline}.

